Dynamic Quantum Key Distribution for Microgrids with Distributed Error Correction

Quantum key distribution (QKD) has often been hailed as a reliable technology for secure communication in cyber-physical microgrids. Even though unauthorized key measurements are not possible in QKD, attempts to read them can disturb quantum states leading to mutations in the transmitted value. Further, inaccurate quantum keys can lead to erroneous decryption producing garbage values, destabilizing microgrid operation. QKD can also be vulnerable to node-level manipulations incorporating attack values into measurements before they are encrypted at the communication layer. To address these issues, this paper proposes a secure QKD protocol that can identify errors in keys and/or nodal measurements by observing violations in control dynamics. Additionally, the protocol uses a dynamic adjacency matrix-based formulation strategy enabling the affected nodes to reconstruct a trustworthy signal and replace it with the attacked signal in a multi-hop manner. This enables microgrids to perform nominal operations in the presence of adversaries who try to eavesdrop on the system causing an increase in the quantum bit error rate (QBER). We provide several case studies to showcase the robustness of the proposed strategy against eavesdroppers and node manipulations. The results demonstrate that it can resist unwanted observation and attack vectors that manipulate signals before encryption.

==> prev_text <==
\subsection{Operating Principle}
\begin{figure}
\centering
\centerline{{\includegraphics[width=0.85\linewidth]{quantum_one.pdf}}}
\caption{{Microgrid control architecture.}}
\label{fig:control}
\end{figure}
Fig. \ref{fig:control} displays a single-line illustration of a cyber-physical DC microgrid network with $N=4$ distributed energy resources (DERs), each coupled with a corresponding DC/DC buck converter {\color{blue} \textbf{Label the 4 DERs in Fig. 1. Current figure labels with DG-$i,j$ is not clear.}}. Each of the DER-converter pairings is also referred to as an \textit{agent}. The set of agents in the microgrid network is physically interconnected via transmission lines and also linked through a communication layer that enables the network elements to exchange data. The data from the communication layer is then processed by each agent's local secondary controller. As illustrated in Fig. \ref{fig:control}, this local control mechanism integrates voltage and current controllers tailored for DC/DC converter operation. In addition, the secondary control mechanism incorporates an average voltage controller to ensure global voltage stabilization and a current controller for even load distribution by applying voltage offsets across each layer.

\begin{figure*}
\centering
\centerline{{\includegraphics[width=0.70\linewidth,clip,trim={0 10 0 21}]{quantum_two.pdf}}}
\caption{Distributed controller for microgrids under consideration in $k^{th}$ DG.}
\label{fig:controlone}
\end{figure*}

In Fig. \ref{fig:control}, an interconnected graph portrays the cyber components in a non-directional fashion. Here, the agents are symbolized by nodes and are represented as $\textbf{x} = \{{x}_1, {x}_2, \ldots, {x}_N\}$. Adjacency relationships between these nodes are represented through edges and an associated adjacency matrix, ${\mathbf A_\text{G}} = [{a}_{kj}]\in{R^{N\times{N}}}$, where the term $a_{kj}$ (indicating a connection from node $j$ to node $k$) holds a value greater than 0 only when ($\psi_k$, $\psi_j$) $\in$ $\mathbf{E}$ (in this formulation, $\mathbf{E}$ signifies an edge representing the connection between two microgrid nodes, with $\psi_k$ being a local node and $\psi_j$ signifying its neighbor). If no cyber link is present between $\psi_k$ and $\psi_j$, then $a_{kj}$ = 0.
Within this configuration, an agent (for example, at the $\psi_k$ node) exchanges local voltage and current statistics with its neighboring nodes denoted as, $N_{k} = \{ {j} \ | \ ({\psi}_j, {\psi}_k) \in \mathbf{E} \} $. The matrices reflecting this input and output data are depicted as $\mathbf{D}_\text{in} = \texttt{diag}\{{d}_k^{in}\}$ and ${\mathbf{D}_\text{out}} = \texttt{diag}\{{d}_k^{out}\}$, where the elements are formulated as ${d}_k^{in}=\sum_{j\in N_{k}}a_{kj}$ and ${d}_k^{out}=\sum_{i\in N_{j}}a_{jk}$ respectively {\color{blue} \textbf{${d}_k^{in}, {d}_k^{out}$} not defined here!}.
The Laplacian matrix (obtained through the combination of sent and received information), described by $\mathbf{L}$ = [${l}_{kj}$], derives its elements from the relationship $\mathbf{L}$ = ${\mathbf{D}_\text{in}} - {\mathbf{A}_\text{G}}$.

The underlying function of the cooperative control system is to ensure consistent global regulation and to facilitate proportional distribution of the load current. For these objectives, two voltage correction terms are utilized to establish the reference voltage, specifically:
\begin{align}
 \Delta V_{1k}(t) &  =K_{P}^{H_1}(V_ {\rm dcref} - \bar{V}_i (t))
+K_{I}^{H_1}\int(V_ { \rm ref}- \bar{V}_k (t))dt
\end{align}
\begin{equation}
\Delta V_{2i}(t)=K_{P}^{H_2}\delta _{k}{ (t)}+K_{I}^{H_2}\int\delta _{k}{ (t)}dt
\end{equation}
In the above equations, $\bar{V}_{i}$ signifies the approximate voltage average for the $i^\text{th}$ agent, ${V}_{\rm ref}$ is the reference voltage, and $\delta _{k}$ is an error signal signifying the discrepancy in per-unit output current for the $k^\text{th}$ agent (in comparison to current measurement signals received from its neighbors).
Outputs from the voltage observer and power-sharing controller, as portrayed in Fig. \ref{fig:controlone} {\color{blue} \textbf{**Missing Figure?**}}, are mathematically described by:
\begin{equation}\label{enq:e1}
\bar{V}_{k}(t)=V_{{k}}(t)+\int \sum _{j\in N_{k}}a_{kj}(\bar{V}_{j}(t-\tau )-\bar{V}_{k}(t-\tau ))dt
\end{equation}
\begin{equation}\label{enq:e2}
\delta _{k}{ (t)}=\sum _{j\in N_{k}}ca_{kj}\left (  \frac{I_{{j}}(t-\tau)}{I_{{j}}^{max}}-\frac{I_{{k}}(t-\tau )}{I_{{k}}^{max}}\right )
\end{equation}
In the above equations, $\tau$ signifies the communication delay between agents, and $c$ denotes the coupling gain. The terms $I_{{k}}$, $I_{{j}}$, $I_{{k}}^{max}$, and $I_{{j}}^{max}$ represent the current values for the respective agents.

For the $k^\text{th}$ agent, the local voltage reference, $V_{k}^{*}$, is derived from the correction terms in (1)-(2) and is expressed as:
\begin{equation}
V_{k}^{*}(t)=V_ { \rm ref}+\Delta V_{1k}(t)+\Delta V_{2k}(t).
\end{equation}
%
In the context of a well-linked cyber graph within the DC microgrid system and under the cooperative consensus algorithm, the macro-level control objectives are defined by:
\begin{equation}\label{enq:e6}
\lim_{k\rightarrow \infty }\bar{V}_{k}(t)=V_{\rm ref},\quad \lim_{k\rightarrow \infty }\delta _{k}(t)=0.\quad\forall k\in N
\end{equation}

\begin{table}
	\renewcommand{\arraystretch}{1.3}
	\caption{Stealth Attacks in DC Microgrids in \cite{sahoo2018stealth} and \cite{sahoo2019detection}}
	\label{tab:1}
	\centering
	\begin{tabular}{c|c}
		\hline
		Affected Counterparts & Modeling \\
		\hline
		\hline
		
		Voltage \cite{sahoo2018stealth} & $\undb{W} {x}^V_{attack}$ = 0 \\
		\hline
		
		Current \cite{sahoo2019detection} & $\undb{W} {x}^I_{attack}$ = 0\\
		\hline
	\end{tabular}
\end{table}

\subsection{Cybersecurity Issues in Generic Microgrids}
Fig. \ref{fig:control} illustrates the potential for malicious actors to introduce deceptive data into the network devices, internet-of-things (IoT) modules, cyber-physical controllers, and other cyber components associated with a weakly encrypted DC microgrid system. This can sabotage the goals specified in (\ref{enq:e6}). Intriguingly, these malevolent activities can be executed in tandem, tricking the microgrid operators by introducing additional, unauthorized parameters into (\ref{enq:e1})-(\ref{enq:e2}). This can be mathematically expressed as:
    \begin{eqnarray}
\undb{u}^{a}(t) = \undb{L} \undb{x}(t) +  \undb{W} \undb{x}_{attack} \label{12}    \end{eqnarray}
In the above equations, $\undb{u}^a$ symbolizes the vector form of the manipulated control input, defined by $u^a_k$ = \{$u^{Va}_k, u^{Ia}_k$\} {\color{blue} \textbf{The notation looks confusing to me..}}.
Furthermore, $\undb{x}_{attack}$ and $\undb{x} = \{ \bar{\undb{V}}, \undb{I}\}$ represent the attack components, detailed as $x_{attack_{i}}$ = [$x^{V}_{attack_{k}}, x^{I}_{attack_{k}}]^T$, and the uncompromised metrics, in that order.
The matrix representing the distribution of attacks, $\undb{W}$ = [$w_{kj}$], displays row-stochastic behavior. Its elements can be detailed as:
\begin{eqnarray}
w_{kj} = {\begin{cases}
	\frac{1}{N_k + 1}, \ j \in N_k\\
	1 - \sum_{j \epsilon N_k} w_{kj}, \ j = k \\
	0, j \not\in N_k, j \neq k
	\end{cases}} \label{14}
\end{eqnarray}
Table \ref{tab:1} provides an insight into stealth attacks, while detection methodologies for these attacks are covered in Table \ref{tab:2}. For a comprehensive understanding, readers can refer to \cite{sahoo2018stealth} and \cite{sahoo2019detection}. A critical observation from Table \ref{tab:2} is that the detection mechanisms are heavily reliant on both local and neighboring metrics. This dependency presents a golden opportunity for malevolent entities to breach the communication metrics essential for devising detection strategies. This can potentially hinder the ability to identify these breaches, especially if the conditions in Table \ref{tab:2} are unfulfilled.
\begin{table}
	\renewcommand{\arraystretch}{1.3}
	\caption{Detection Criteria for Stealth Attacks in Table \ref{tab:1}}
	\label{tab:2}
	\centering
\begin{threeparttable}
	\begin{tabular}{c|c|c}
		\hline
		Stealth Attack & Detection Criteria for $k^{th}$ Agent & Terminology \\
		\hline
		\hline
		
		Voltage \cite{sahoo2018stealth} & \begin{tabular}{@{}c@{}} $h_k$\tnote{1} $[\sum_{j \epsilon N_k} a_{kj} (\Delta V_{1_{j}} - \Delta V_{1_{k}})]$\\ $[\sum_{j \epsilon N_i} a_{kj} (\Delta V_{1_{j}} + \Delta V_{1_{k}})] >$  $\Upsilon_1$ \end{tabular}& $DM^k_1$ \\
		\hline
		
		Current \cite{sahoo2019detection} & \begin{tabular}{@{}c@{}} $c_k [\sum_{j \epsilon N_k} a_{kj} (I^{j}_{in_{ref}} - I^{k}_{in_{ref}})]$\\ $[\sum_{j \epsilon N_k} a_{kj} (I^{j}_{in_{ref}} + I^{k}_{in_{ref}})] >$  $\Upsilon_2$ \end{tabular}\tnote{2} & $DM^k_2$\\
		\hline
	\end{tabular}
  \begin{tablenotes}
	\item[1] $h_k$ is a positive quantity used for $i^{th}$ agent.
	\item[2] $c_k$ is another positive quantity. $I^{k}_{in_{ref}}$ represents the value of input current reference for the $k^{th}$ agent.
\end{tablenotes}
\end{threeparttable}
\end{table}
A major requirement for attackers to execute a successful stealth attack is that they should be able to eavesdrop on the communication channels associated with the microgrid network and learn system information \cite{rath2022behind}. This is generally possible if the communication network uses a weak cryptographic protocol.


==> usepackage.tex <==
\usepackage{times}
\usepackage{amsmath,epsfig}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{array,dcolumn}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{subcaption}
\usepackage{psfrag}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{balance}
\usepackage{accents}
\usepackage{booktabs, adjustbox}
\usepackage{cite}
\usepackage[all]{xy}
\interdisplaylinepenalty=2500
\usepackage{dsfont}
\usepackage{hyperref}
\usepackage{url}
\usepackage{xcolor}
\usepackage[nolist]{acronym}
\usepackage{graphicx}
\usepackage{float}
\usepackage{threeparttable}
\usepackage{cancel}
\usepackage[official]{eurosym}
\usepackage{chemformula}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{comment}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{multibib}

\usepackage{xcolor}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{mathtools,amssymb,lipsum, nccmath}
\usepackage{cuted}

\newcommand{\LD}[1]{\textcolor{blue}{#1}}

\def\undb#1{\mbox{\bf{#1}}}

\include{pythonlisting}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}


\hypersetup{
     colorlinks = false,
     linkcolor = black,
     anchorcolor = black,
     citecolor = black,
     filecolor = blue,
     urlcolor = black
     }

\hyphenation{op-tical net-works semi-conduc-tor}


